Replication-Robust Payoff-Allocation for Machine Learning Data Markets

Submodular functions have been a powerful mathematical model for a wide range of real-world applications. Recently, submodular functions are becoming increasingly important in machine learning (ML) for modelling notions such as information and redundancy among entities such as data and features. Among these applications, a key question is payoff allocation, i.e., how to evaluate the importance of each entity towards the collective objective? To this end, classic solution concepts from cooperative game theory offer principled approaches to payoff allocation. However, despite the extensive body of game-theoretic literature, payoff allocation in submodular games are relatively under-researched. In particular, an important notion that arises in the emerging submodular applications is redundancy, which may occur from various sources such as abundant data or malicious manipulations where a player replicates its resource and act under multiple identities. Though many game-theoretic solution concepts can be directly used in submodular games, naively applying them for payoff allocation in these settings may incur robustness issues against replication. In this paper, we systematically study the replication manipulation in submodular games and investigate replication robustness, a metric that quantitatively measures the robustness of solution concepts against replication. Using this metric, we present conditions which theoretically characterise the robustness of semivalues, a wide family of solution concepts including the Shapley and Banzhaf value. Moreover, we empirically validate our theoretical results on an emerging submodular ML application, i.e., the ML data market.

==> sections/algorithm.tex <==

\begin{algorithm}[t]
	\caption{Sampling Algorithm for Semivalues}
	\label{algo:stratified_group_testing}
	\begin{algorithmic}[1]
		\Statex{\textbf{Input:} T: number of samples, $N$: the set of players, $q(c)$: any sampling distribution over coalition sizes $c$, $\alpha_c$, importance weights of the semivalue $\varphi$.}
		\Statex{\textbf{Output:} estimated payoff value $\hat{\varphi}'_i$ of each player}
		%\STATE{Initialize empty sets $U_i^+(c), U_i^-(c)$ for players $i\in N, c= 0,1,...,N$}
		\State{\text{\textbf{Step 1: Sampling coalitions and computing utilities}}}
		\For{$t=1,2,\ldots T$} 
		\State{Draw coalition size $c_t \sim q(c)$}
		\State{Uniformly sample coalition $\S_t \subseteq N$ of size $c_t$}
		\State{Compute $v(\S_t)$}
		%\STATE{Add $v(S_t)$ to sets $U_i^+(\medmath{c_t-1})$, $U_i^-(\medmath{c_t})$ for $i \in S_t$}
		\EndFor
		\State{$U_c \leftarrow \frac{1}{||\S_t|=c|}\sum_{|\S_t|=c} v(\S_t)$ for all $c$}
		\State{$\Bar{U}_i(c) \leftarrow \frac{1}{||\S_t|=c, i\in \S_t|}\sum_{|\S_t|=c, i\in \S_t} v(\S_t)$ for all $c$ and $i$}
        \State{\text{\textbf{Step 2: Approximating players' values}}}
		%\STATE{$\Bar{U}_i^- \leftarrow \tfrac{1}{|U_i^-|} \sum_{u \in U_i^-} u$; $\Bar{U}_i^+ \leftarrow \tfrac{1}{|U_i^+|} \sum_{u \in U_i^+} u$ } 
		\State{$\hat{\varphi}_i \leftarrow \sum_{c=0}^{N-1}\alpha_c  \frac{N}{N-c}(\tfrac{N-c}{N} \Bar{U}_i(c+1) + \frac{c}{N} \Bar{U}_i(c)- U_c)$}
		\State{Compute players' pairwise differences $\Delta \hat{\varphi}_{ij} \leftarrow \hat{\varphi}_i - \hat{\varphi}_j$,}
		\State{Compute approximated total payoff $\hat{\varphi}_\textnormal{all} \leftarrow N\sum_{c=0}^{N-1}\alpha_c (U_{c+1} - U_c)$} 
		\State{Find $\hat{\varphi}'_i$ by solving a feasibility program with the following constraints:\\  $\sum_i{\hat{\varphi}'_i} = \hat{\varphi}_\textnormal{all}$, $|(\hat{\varphi}'_i - \hat{\varphi}'_j) - \Delta \hat{\varphi}_{ij}| \leq \epsilon$ for $\forall i,j\in N$} 
	\end{algorithmic} 
\end{algorithm}


==> sections/algorithm_oracle.tex <==
\begin{figure*}[t]
\begin{minipage}{0.5\linewidth}
	\begin{algorithm}[H]
	\begin{algorithmic}[1]
		\Statex{\textbf{Input:} $N$: the set of all players}
		\Statex{\textbf{Output:} $v:2^N\rightarrow \mathbb{R}$: characteristic function of all possible coalitions of the players}
		\For{coalition $\S\subseteq N$}
		    \State{$\mu \leftarrow 0.01 \sum_{i\in \S} i$}
		    \State{$\sigma\leftarrow 0.05$}
		    \State{Assign utility to the coalition}
		    \State{$v(\S) \leftarrow (1-e^{-|\S|}) + \mathcal{N}(\mu , \sigma^2)$}
		\EndFor
	\end{algorithmic} 
	\captionof{algorithm}{Random Set Function} 
	\label{algo:oracle}
	\end{algorithm}
\end{minipage}
\begin{minipage}{0.5\linewidth}
	\centering
	\includegraphics[width=0.6\linewidth]{market/img/zc/zc_oracle.pdf}
	\captionof{figure}{Avg. marginal contributions $z_i(c)$ for the random set function}
	\label{fig:zc_oracle}
\end{minipage}
\end{figure*}


==> sections/efficient.tex <==
\subsection{Efficient Computation}\label{sec:sampling}

Due to the combinatorial nature of game-theoretic solution concepts, computing the payoff-allocation requires the characteristic values of all possible coalitions, which is exponential on the number of players and often very computationally expensive. For more efficient computation, we may sometimes obtain closed-form solutions, such as in Section~\ref{app_sub:facility_location}, where we derived closed-form solutions and efficient algorithms for computing the Shapley value and the Banzhaf value in facility location games. 

However, in more real-life applications such as the data market, a closed-form expression of the characteristic function is usually absent and hence no closed-form solution concepts are possible. In particular, the computation of the semivalues in the data market game is very demanding, as it requires the evaluation of $v(\cdot)$ for a large number of coalitions, each involving the training of ML models.
As this quickly becomes infeasible, methods for approximating the solution concepts are crucial.
In this section, we draw inspirations from prior sampling methods, and introduce a novel sampling algorithm which efficiently approximates the semivalues.

\subsubsection{Prior Works}
Prior approximation methods~\cite{fatima2008linear, bachrach2008approximating} mainly focused on the Shapley value and specific types of cooperative games such as weighted voting games. In the following we list a few important approximation methods that are relevant to our problem setting.

\emph{Random (Permutation) Sampling}~\cite{castro2009polynomial, agarwal2019marketplace}. This is one of the most common methods for approximating the Shapley value. The method samples $T$ permutations $\pi^t$ of players, iteratively computes the marginal contribution $\mc^t_{i}$ of each player $i$ towards the preceding players in $\pi^t$, and approximates the Shapley value of each player by averaging over the samples $\hat{\varphi}^{shapley}_i = \frac{1}{T}\sum_t{\mc^t_{i}}$.

\emph{Stratified Sampling}~\cite{maleki2013bounding}. This method is a stratified refinement that 
approximates for each player the average marginal contributions $z_i(c)$ over size-$c$ coalitions, and then computes the Shapley value by averaging over $z_i(c)$'s. Though the original paper~\cite{maleki2013bounding} focused on the Shapley value, we observe that this method can be extended to approximate semivalues.

\emph{Group Testing}~\cite{jia2019towards}. This is a more recent method developed for approximating the Shapley value. In particular, this method effectively shares sampled coalitions among players. In each turn $t$, it draws a coalition $\S_t$ of a sampled size $k_t$. After drawing the coalitions, the method proceeds by estimating players' pairwise differences $\Delta \hat{\varphi}_{ij} \propto \sum_t(\mathbbm{1}_{i\in \S_t}-\mathbbm{1}_{j\in \S_t})v(\S_t)$, and by using the sum of their values $v(N)$, the approximate Shapley value can be obtained via solving a feasibility program.

Among the above methods, random sampling and group testing cannot be used to approximate solution concepts beyond the Shapley value: the former performs uniform permutation sampling, and the latter requires the total allocated payoff, which can only be efficiently obtained for the Shapley value as $v(N)$ by the Efficiency Axiom~\ref{ax:efficiency}). 
Stratified sampling can be extended beyond the Shapley value through Equation~\ref{eq:zc}, however, with a growing number of players, separate assignment of samples to players can be suboptimal.


\subsubsection{A Sampling Algorithm for Semivalues}
Motivated by the above considerations, we propose a novel sampling algorithm (Algorithm~\ref{algo:stratified_group_testing}) which applies to any semivalue as defined by Equation~\ref{eq:zc}. By rewriting the players' average marginal contributions, our algorithm improves the sample efficiency of stratified sampling by enabling sample sharing among the players. Furthermore, by approximating the total payoff, our algorithm extends to solution concepts beyond the Shapley value to all semivalues. The next theorem provides two unbiased estimators for the payoff of each player and the total payoff for all players.

\begin{restatable}{theorem}{approxvalues}
	\label{thm:approx_payoff}
	Let $G=(N, v)$ be a market game and a semivalue defined as $\varphi_i=\sum_{c=0}^{N-1}\alpha_c z_i(c)$, Algorithm~\ref{algo:stratified_group_testing} provides unbiased estimators  $\hat{\varphi_i} = \sum_{c=0}^{N-1}\alpha_c \tfrac{N}{N-c} [\tfrac{N-c}{N}\Bar{U}_i(c+1) + \tfrac{c}{N}\Bar{U}_i(c) - U_c]$ for the payoff of all players $i$, and 
    $\hat{\varphi_\textnormal{all}} = N\sum_{c=0}^{N-1}\alpha_c (U_{c+1} - U_c).$ for total payoff allocated to all players, where $U_c$ is the mean of size $c$ coalitions, and $\bar{U}_i(c)$ is the mean of size $c$ coalitions which contain player $i$.
\end{restatable}
\begin{proof}
For the proof please refer to the appendix
\end{proof}

\input{sections/algorithm.tex}
Algorithm \ref{algo:stratified_group_testing} works as follows:
It first samples coalitions according to a distribution $q(c)$ over coalition size $c$, then approximates the payoff of each player according to the estimator from Theorem~\ref{thm:approx_payoff}, $\hat{\varphi}_i =\sum_{c=0}^{N-1}\alpha_c  \frac{N}{N-c}(\tfrac{N-c}{N} \Bar{U}_i(c+1) + \frac{c}{N} \Bar{U}_i(c)- U_c)$, where $\Bar{U}_i(c)$ is the average value of sampled size-$c$ coalitions that contain player $i$, and $U_c$ is the average value of all sampled coalitions of size $c$.
Next, we compute the players' pairwise differences. Finally, we compute the estimated payoff of each player through a feasibility program which makes use of the players' pairwise differences and the approximated total allocated payoff $\hat{\varphi}_\textnormal{all} \leftarrow N\sum_{c=0}^{N-1}\alpha_c (U_{c+1} - U_c)$.
The feasibility program is formulated as follows and can be solved using existing software such as the Python PuLP package:
\begin{alignat*}{2}
  \mathop{\textrm{minimize}}_{\hat{\varphi}_1', \ldots, \hat{\varphi}_N'} \quad &   0 & \\
   \textrm{subject to} \quad & \begin{aligned}[t] \sum_{i=1}^{N}
                    \hat{\varphi}'_{i}  =\hat{\varphi}_{all} &\\[3ex]
                  \hat{\varphi}'_{i} - \hat{\varphi}'_{j} - \Delta \hat{\varphi}_{ij} &\leq \epsilon , & \quad i,j &=1 ,\dots, N\\[3ex]
                  \hat{\varphi}'_{i} - \hat{\varphi}'_{j} - \Delta \hat{\varphi}_{ij} &\geq -\epsilon , & \quad i,j &=1 ,\dots, N
                \end{aligned}
\end{alignat*}

\iffalse
The feasibility program is inspired by the group testing approach. In the small sample regime, i.e., when the samples provide insufficient coverage of the different coalition sizes, the feasibility program can help adjust the estimates by adding a sum constraint over the payoff of all players and thereby interpolating the values among the players.
\begin{figure}[h]
	\centering
	\begin{minipage}{\linewidth}
	\centering
	\includegraphics[width=0.7\linewidth, height=0.3cm]{market/img/sampling/covertype/sampling_legend.pdf}
	\subfloat[Before Step 3]{\includegraphics[width=0.4\linewidth]{market/img/feasibility_demo/shapley_non_gt.pdf}\label{fig:before_feasibility}}%
	\subfloat[After Step 3]{\includegraphics[width=0.4\linewidth]{market/img/feasibility_demo/shapley_gt.pdf}\label{fig:after_feasibility}}
	\end{minipage}\vfill
	\begin{minipage}{\linewidth}
	\centering
	\subfloat[Count of each player in the sampled coalitions]{\includegraphics[width=0.9\linewidth, height=0.4\linewidth]{market/img/feasibility_demo/count.pdf}\label{fig:count_feasibility}}%
	\end{minipage}
	\caption{Example effect of applying the feasibility program.}
	\label{fig:feasibility_demo}
\end{figure}
Figure~\ref{fig:feasibility_demo} illustrates this effect %on the experiment \emph{Uniform} 
for approximating the Shapley value of an $8$ player market game. More details about the market games are in the experiments section.
Specifically, Figures~\ref{fig:before_feasibility} and~\ref{fig:after_feasibility} show the approximated Shapley values as compared with the ground truth using Algorithm~\ref{algo:stratified_group_testing} before and after applying the feasibility program. 
In Figure~\ref{fig:before_feasibility} with 32 samples, the estimated Shapley values of players $1,2,3,4$ are far below the true Shapley value.
With the feasibility program, each player's value is interpolated from other players' values, as shown in Figure~\ref{fig:after_feasibility}.
Figure~\ref{fig:count_feasibility} shows the coverage of the sampled coalition sizes for each player for sample size $32$ and $64$. For sample sizes of $32$, some coalition sizes are not covered, and interpolation using the feasibility program helps reduce the negative effect.
The sampling algorithm reduces the number of characteristic value evaluations from $2^N$ to the number of samples. All other calculations incur negligible time. Orthogonal to a sampling based approach, approximations to the characteristic values $v(\S)$ can be applied to further improve efficiency, and would be an interesting direction for future work.
\fi

==> sections/sampling_table.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table*}[t]
\centering
\caption{Relative error of the sampling algorithms. Bold font indicates best result for each dataset and number of samples.}
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}cccccccccc@{}}
\toprule
 &  & \multicolumn{2}{c}{\textbf{Random Sampling}} & \multicolumn{2}{c}{\textbf{Stratified Sampling}} & \multicolumn{2}{c}{\textbf{Group Testing}} & \multicolumn{2}{c}{\textbf{Ours}} \\ \cmidrule(l){2-10} 
 & \textit{\textbf{\# samples}} & \textit{\textbf{64}} & \textit{\textbf{128}} & \textit{\textbf{64}} & \textit{\textbf{128}} & \textit{\textbf{64}} & \textit{\textbf{128}} & \textit{\textbf{64}} & \textit{\textbf{128}} \\ \midrule
\multirow{3}{*}{\textbf{Covertype}} & \textit{Shapley} & $0.93\pm 0.16$ & $0.63\pm 0.11$ & $1.30\pm0.86$ & $0.89\pm 0.32$ & $2.98\pm0.26$ & $2.04\pm0.46$ & $\boldsymbol{0.06\pm0.02}$ & $\boldsymbol{0.04\pm0.01}$ \\ %\cmidrule(l){2-10} 
 & \textit{Banzhaf} & - & - & $0.66\pm0.23$ & $0.53\pm0.10$ & - & - & $\boldsymbol{0.31\pm0.12}$ & $\boldsymbol{0.25\pm0.11}$ \\ %\cmidrule(l){2-10} 
 & \textit{Robust Shapley} & - & - & $0.41\pm0.20$ & $0.30\pm0.12$ & - & - & $\boldsymbol{0.24\pm0.07}$ & $\boldsymbol{0.23\pm0.08}$ \\ \midrule
\multirow{3}{*}{\textbf{CIFAR-100}} & \textit{Shapley} & $0.23\pm 0.12$ & $0.16\pm 0.06$ & $0.30\pm 0.14$ & $0.22\pm 0.11$ & $1.08\pm 0.44$ & $0.67\pm 0.28$ & $\boldsymbol{0.13\pm 0.05}$ & $\boldsymbol{0.08\pm 0.03}$ \\ %\cmidrule(l){2-10} 
 & \textit{Banzhaf} & - & - & $0.31\pm 0.24$ & $0.27\pm 0.25$ & - & - & $\boldsymbol{0.20\pm 0.10}$ & $\boldsymbol{0.10\pm 0.04}$ \\ %\cmidrule(l){2-10} 
 & \textit{Robust Shapley} & - & - & $0.26\pm 0.15$ & $0.16\pm 0.08$ & - & - & $\boldsymbol{0.19\pm 0.09}$ & $\boldsymbol{0.11\pm 0.04}$ \\ \midrule
\multirow{3}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Tiny \\ ImageNet\end{tabular}}} & \textit{Shapley} & $0.38\pm0.14$ & $0.24\pm0.12$ & $0.44\pm0.19$ & $0.24\pm0.15$ & $1.34\pm0.39$ & $0.91\pm0.29$ & $\boldsymbol{0.12\pm0.06}$ & $\boldsymbol{0.09\pm0.03}$ \\ %\cmidrule(l){2-10} 
 & \textit{Banzhaf} & - & - & $0.63\pm0.39$ & $0.53\pm0.22$ & - & - & $\boldsymbol{0.42\pm0.12}$ & $\boldsymbol{0.26\pm0.09}$ \\ %\cmidrule(l){2-10} 
 & \textit{Robust Shapley} & - & - & $0.88\pm0.46$ & $0.67\pm0.35$ & - & - & $\boldsymbol{0.60\pm0.16}$ & $\boldsymbol{0.38\pm0.16}$\\
 \midrule
%
\multirow{3}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Random Function \\ \end{tabular}}} & \textit{Shapley} & $0.46\pm0.11$ & $0.36\pm0.07$ & $0.40\pm0.21$ & $0.21\pm0.15$ & $2.00\pm0.35$ & $1.40\pm0.33$ & $\boldsymbol{0.12\pm0.02}$ & $\boldsymbol{0.08\pm0.02}$ \\ %\cmidrule(l){2-10} 
& \textit{Banzhaf} & - & - & $1.06\pm0.45$ & $0.69\pm0.20$ & - & - & $\boldsymbol{0.51\pm0.50}$ & $\boldsymbol{0.23\pm0.05}$ \\ %\cmidrule(l){2-10} 
& \textit{Robust Shapley} & - & - & $1.09\pm0.38$ & $0.83\pm0.16$ & - & - & $\boldsymbol{0.50\pm0.20}$ & $\boldsymbol{0.28\pm0.09}$ \\
\midrule
%
\multirow{3}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Facility Location \\ \end{tabular}}} 
& \textit{\textbf{\# samples}} & \multicolumn{1}{c}{\textbf{\emph{256}}}& & \multicolumn{1}{c}{\textbf{\emph{256}}}& & \multicolumn{1}{c}{\textbf{\emph{256}}}& & \multicolumn{1}{c}{\textbf{\emph{256}}}&\\ %\cmidrule(l){2-10} 
& \textit{Shapley $\medmath{(\!N\!=\!128)}$} & \multicolumn{1}{c}{$1.57\pm 0.04$} & & \multicolumn{1}{c}{$0.95\pm 0.06$} & & \multicolumn{1}{c}{$57.3\pm 6.61$} & &\multicolumn{1}{c}{$\boldsymbol{0.08\pm 0.002}$} &\\ %\cmidrule(l){2-10} 
& \textit{Banzhaf $\medmath{(\!N\!=64)}$} & \multicolumn{1}{c}{-}& &  \multicolumn{2}{c}{$1.59\pm 0.99$ ($\varphi_\textnormal{all}$ $14.99\pm 0.99$)} &  \multicolumn{1}{c}{-} & & \multicolumn{2}{c}{$\boldsymbol{0.72\pm 0.10}$ ($\varphi_\textnormal{all}$ $\boldsymbol{0.40\pm 0.02}$)} \\
\bottomrule
\end{tabular}%
}
\label{table:sampling}
\end{table*}

==> sections/supermodular.tex <==

\iffalse 
\subsection{Generalisation to Supermodular Games}\label{sec:generalise}

Though our main focus of the chapter is on submodular games and total payoffs of replicating players, the framework can be generalised to supermodular games, and our theoretical results can be extended to study related metrics and more complex manipulations. 
In this section, we discuss some of the potential generalisations of our theoretical results to supermodular games and alternative manipulation scenarios related to replication. 

\subsubsection{Supermodular Games}
\label{sec:supermodular}
%
In this section, We extend some of our theoretical results to supermodular games, i.e., characteristic function games with supermodular and replication-redundant characteristic functions. Compared with the submodular case, Lemma~\ref{lemma:zc_supermodular} shows that the average marginal contributions $z_i(c)$ increases with coalition size, Theorem~\ref{thm:robustness_condition_supermodular} states the condition for replication-robustness, and Theorem~\ref{thm:gain_decrease} discusses the behaviours of common solution concepts.

\begin{restatable}{lemma}{zcsupermodular}\label{lemma:zc_supermodular}
Given a supermodular characteristic function, the average marginal contribution $z_i(c)$ monotonic increases with coalition size $c$:\\
\centerline{$\forall {0\leq c < N-1}, \quad z_i(c) \leq z_i(c+1).$}
\end{restatable}
\begin{proof}[Proof Sketch:]
To prove this lemma, we substitute the submodularity condition by supermodularity in the proof of Lemma~\ref{lemma:zc_monotone}, i.e., $\S_1 \subseteq \S_2\subseteq N\setminus\{i\} \implies \mc_i(\S_1) \leq \mc_i(\S_2)$, which then compares $z_i(c)$ and $z_i(c+1)$ by matching the size-$c$ coalitions with their size-$(c+1)$ supersets.
\end{proof}
The next example illustrates the changes in the total payoff of the replicating player:
\begin{example}\label{example:alpha_ck_supermodular}
Let $G = (N, v)$ be a supermodular game with 3 players $N=\{i, p, q\}$. The marginal contributions of player $i$ are $\mc_i(\emptyset) = 1$, $\mc_i(\{p\})= \mc_i(\{q\}) = 2$, $\mc_i(\{p,q\}) = 3$. Player $i$ replicates once and acts under two identities $\S^R = \{i_1, i_2\}$. The induced game is $G^R = (N^R, v^R)$ where $N^R = \{i_1, i_2, p, q\}$, and $v^R$ satisfies $\forall \S\subseteq \{p, q\}, v^R(\{i_1\}\cup \S) = v^R(\{i_2\}\cup \S) = v(\{i\}\cup \S)$. \\
\noindent
(1) The average marginal contributions of player $i$ in the original game are:\\
\centerline{$z_i(0) = \mc_i(\emptyset) = 1; \quad  z_i(1) = \frac{1}{2} (\mc_i(\{p\})+ \mc_i(\{q\}))= 2; \quad z_i(2) =\mc_i(\{p,q\})= 3.$}
\noindent
(2) Importance weights in the induced game according to Equation~\eqref{eq:alpha_ck}: 

(Shapley) $\weight{c}{N+k} \coloneqq \tfrac{1}{N+k}\tbinom{N+k-1}{c}^{-1} \implies \alpha_c^k = \frac{k+1}{N+k}\tbinom{N-1}{c}\tbinom{N+k-1}{c}^{-1},$

(Banzhaf) $\weight{c}{N+k} \coloneqq \tfrac{1}{2^{N+k-1}} \phantom{----,}\implies \alpha_c^k = \frac{k+1}{2^{N+k-1}}\tbinom{N-1}{c}$.

\noindent
(3) The total payoffs of player $i$ is $\varphi_i^\textnormal{tot}(k) = \sum_{c=0}^{N-1}\alpha_c^k z_i(c)$, where $k=0$ refers to before replication: 

(Shapley)
\phantom{-}$\varphi_i^\textnormal{tot}(k=0) = \tfrac{1}{3}(1+2+3) = 2;$ \phantom{------------}
$\varphi_i^\textnormal{tot}(k=1) = 1\cdot\tfrac{1}{2}+2\cdot\tfrac{1}{3}+ 3 \cdot \tfrac{1}{6} = \tfrac{5}{3}$.

(Banzhaf)
$\varphi_i^\textnormal{tot}(k=0) =1 \cdot \tfrac{1}{4}+2 \cdot \tfrac{1}{2}+ 3 \cdot \tfrac{1}{4} = 2;$ \phantom{-----.}
$\varphi_i^\textnormal{tot}(k=1) = 1 \cdot \tfrac{1}{4}+2\cdot \tfrac{1}{2}+ 3 \cdot \tfrac{1}{4} = 2.$
\end{example}
Compared with the submodular game in Example~\ref{example:alpha_ck}, here the player $i$'s total payoff decreases after replication under the Shapley value, which is opposite to the submodular case, whereas for the Banzhaf value, the total payoff of player $i$ stays invariant with the first replication for both cases.
The next theorem presents the condition for replication-robustness properties for supermodular games.
\begin{restatable}{theorem}{robustnessConditionSupermodular}
\label{thm:robustness_condition_supermodular} 
Let $G= (N, \cv)$ be a supermodular game with replication-redundant characteristic function. A solution concept of the form $\varphi_i = \sum_{c=0}^{N-1}\alpha_c z_i(c)$ 
is replication-robust \emph{iff} for any number of replicas $k$,
\begin{equation}\label{eq:robustness_condition_supermodular}
\forall 0\leq p\leq N-1, \sum_{c=p}^{N-1}\alpha_c^0 \geq \sum_{c=p}^{N-1}\alpha_c^{k},
\end{equation}
where $\alpha_c^k$ is as defined in Equation~\eqref{eq:alpha_ck}.
\end{restatable}
\begin{proof}[Proof Sketch:]
Given monotonic increasing average marginal contributions $z_i(c)$, the theorem can be shown in a similar way as theorem~\ref{thm:robustness_condition} for submodular characteristic functions. 
\end{proof}

\begin{restatable}[]{theorem}{shapleysupermodular}
\label{thm:gain_decrease}
Let $G=(N,\cv)$ be a supermodular game with replication-redundant characteristic function, the Shapley value, Banzhaf value and Leave-one-out are replication-robust.
For Shapley value, the total payoff of the replicating player monotonic decreases over number of replicas, and converges to $i$'s characteristic value, i.e.,
    $\lim_{k\rightarrow{\infty}}\varphi^\textnormal{tot}_{i}(k) = v(\{i\}).$ For Banzhaf and LOO, $\lim_{k\rightarrow{\infty}}\varphi^\textnormal{tot}_{i}(k) = 0.$
\end{restatable}
\begin{proof}[Proof Sketch:]
For the Shapley value, we have shown in Lemma~\ref{lemma:sum_alpha_properties} that the for any number of replications $k$, the importance weights satisfy both Equation~\eqref{subeq:efficiency} $\sum_{c=0}^{N-1} \alpha_c^k = 1$, and Equation~\eqref{subeq:monotonicity}, $\forall p, \sum_{c=0}^{p} \alpha_c^k \leq \sum_{c=0}^{p} \alpha_c^{k+1}$, which together implies $\forall p, \sum_{c=p}^{N-1} \alpha_c^k \geq \sum_{c=p}^{N-1} \alpha_c^{k+1}$. Hence by Theorem~\ref{thm:robustness_condition_supermodular}, the Shapley value is replication-robust. The monotonicity part can be shown in a similar way as Corollary~\ref{thm:monotonicity_condition_shapley}. For the proof of Banzhaf value and leave-one-out, we have shown in the proof of theorem~\ref{thm:gain_increase} that $\forall c, k, \alpha_c^k \geq \alpha_c^{k+1}$, hence they also satisfy Theorem~\ref{thm:robustness_condition_supermodular} and are thus replication-robust.
\end{proof}

\fi





==> sections/table_data_assignments.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table*}[t]
\small
\centering
%\setlength\heavyrulewidth{0.2ex}
%\setlength\extrarowheight{2.5pt}
\caption{Experimental settings for CIFAR-100: training and validation data assignments. %The \emph{Combination} experiment uses 5 random superclasses $C_\textnormal{sup}$, each containing 4 subclasses $C_\textnormal{sub}$. All players are honest, each two hold training data of the same superclass $C_\textnormal{sup}$ but different subclasses. 
The \emph{Uniform, Disjoint, Mixed} experiments use all 20 superclasses and their 100 subclasses. Players 1-4 are honest players while 5-7 are replicas that hold the same data as malicious player 0.}
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}ccccccc@{}}
\toprule
 & \textbf{N} & \textbf{Superclass $C_\textnormal{sup}$} & \textbf{Subclass $C_\textnormal{sub}$} & \textbf{Training Data Assignment} & \textbf{Validation Task} & \textbf{Validation Datasets} \\ \midrule

%\multirow{2}{*}{\textbf{Combination}} & \multirow{2}{*}{10} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}$1-5$\\ (Random)\end{tabular}} & \multirow{2}{*}{4 $C_\textnormal{sub}$ per $C_\textnormal{sup}$} & \multirow{2}{*}{Each player assigned 2 $C_\textnormal{sub}$ of the same $C_\textnormal{sup}$} & \multirow{2}{*}{Predict $C_\textnormal{sup}$} & \multirow{2}{*}{Combinations of $C_\textnormal{sup}$s' validation data} \\
% &  &  &  &  &  &  \\ \midrule
 
    \multirow{2}{*}{\textbf{Uniform}} & \multirow{2}{*}{8} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}20\\ (All)\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}5 $C_\textnormal{sub}$ per $C_\textnormal{sup}$\\ (All)\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Players $0-4$ assigned data from 100 $C_\textnormal{sub}$ uniformly\\ Players (replicas) $5-7$ assigned the same data as Player $0$\end{tabular}} & \multirow{2}{*}{Predict $C_\textnormal{sub}$} & \multirow{2}{*}{All $C_\textnormal{sub}$s' validation data} \\
 &  &  &  &  &  &  \\ \midrule

\multirow{2}{*}{\textbf{Disjoint}} & \multirow{2}{*}{8} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}20\\ (All)\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}5 $C_\textnormal{sub}$ per $C_\textnormal{sup}$\\ (All)\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Players $0-4$ each assigned 20 $C_\textnormal{sub}$\\ Players (replicas) $5-7$ assigned the same data as Player $0$\end{tabular}} & \multirow{2}{*}{Predict $C_\textnormal{sub}$} & \multirow{2}{*}{All $C_\textnormal{sub}$'s validation data} \\
 &  &  &  &  &  &  \\ \midrule
 
\textbf{Mixed} & 8 & \begin{tabular}[c]{@{}c@{}}20\\ (All)\end{tabular} & \begin{tabular}[c]{@{}c@{}}5 $C_\textnormal{sub}$ per $C_\textnormal{sup}$\\ (All)\end{tabular} & \begin{tabular}[c]{@{}c@{}}Players $0-4$ assigned varied portions of each $C_\textnormal{sub}$\\ Players (replicas) $5-7$ assigned the same data as Player $0$\end{tabular} & Predict $C_\textnormal{sub}$ & All $C_\textnormal{sub}$s' validation data \\ 
\bottomrule
\end{tabular}%
}
\label{table:settings}
\end{table*}
